Omnivision forecasting: combining satellite observations with sky images for improved intra-hour solar energy predictions

Integration of intermittent renewable energy sources into electric grids in large proportions is challenging. A well-established approach aimed at addressing this difficulty involves the anticipation of the upcoming energy supply variability to adapt the response of the grid. In solar energy, short-term changes in electricity production caused by occluding clouds can be predicted at different time scales from all-sky cameras (up to 30-min ahead) and satellite observations (up to 6h ahead). In this study, we integrate these two complementary points of view on the cloud cover in a single machine learning framework to improve intra-hour (up to 60-min ahead) irradiance forecasting. Both deterministic and probabilistic predictions are evaluated in different weather conditions (clear-sky, cloudy, overcast) and with different input configurations (sky images, satellite observations and/or past irradiance values). Our results show that the hybrid model benefits predictions in clear-sky conditions and improves longer-term forecasting. This study lays the groundwork for future novel approaches of combining sky images and satellite observations in a single learning framework to advance solar nowcasting.

==> figures.tex <==

\section{Qualitative comparative analysis of the impact of image input on probabilistic predictions}
\label{section:image_input}
\setcounter{figure}{0}
\setcounter{table}{0}


\begin{figure*}[ht!] %[H]%[ht!]%[h!] 
\centering


\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_no_sky_sat_37lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_no_sky_sat_i_37lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

\vspace{-1\baselineskip}
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_no_sat_37lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_no_sat_i_37lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

\vspace{-1\baselineskip}
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_sat_37lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_sat_i_37lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

%\vspace{-1.2\baselineskip}
\caption{Probabilistic prediction curves for different input data (26/05/2019):  sky images, satellite observations and extra irradiance channels (IC). Without the exrta IC (left column), the model based on satellite images only (first raw) outputs the most uncertain predictions, the 5-95\% quantile area ranging from 200 to 1000 W/$\text{m}^2$. Adding an additional IC appears to narrow the predicted uncertainty in the first two setups (sky or satellite images). In addition, models trained on sky images (with or without satellite images or IC) provide the most accurate very short-term prediction (10-min ahead).}

\label{fig:uncertainties_comparisons}
\end{figure*}


\begin{figure*}[ht!] %[H]%[ht!]%[h!] 
\centering

\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_no_sky_sat_37lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_no_sky_sat_i_37lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

\vspace{-1\baselineskip}
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_no_sat_37lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_no_sat_i_37lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

\vspace{-1\baselineskip}
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_sat_37lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190521_sky_sat_i_37lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

%\vspace{-1.2\baselineskip}
\caption{Probabilistic prediction curves for different input data (22/05/2019):  sky images, satellite observations and extra irradiance channels (IC). Without the exrta IC (left column), the model based on satellite images only (first raw) outputs the most uncertain predictions, the 5-95\% quantile area ranging from 200 to 1000 W/$\text{m}^2$. Adding an additional IC appears to narrow the predicted uncertainty in the first two setups (sky or satellite images). In addition, models trained on sky images (with or without satellite images or IC) provide the most accurate very short-term prediction (10-min ahead).}

\label{fig:uncertainties_comparisons}
\end{figure*}


\begin{figure*}[ht!] %[H]%[ht!]%[h!] 
\centering

\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190522_no_sky_sat_38lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190522_no_sky_sat_i_38lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

\vspace{-1\baselineskip}
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190522_sky_no_sat_38lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190522_sky_no_sat_i_38lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

\vspace{-1\baselineskip}
\begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190522_sky_sat_38lf.png}
  \end{minipage} 
  %\quad
  \begin{minipage}[b]{0.48\textwidth}
    \includegraphics[width=1.0\textwidth]{Figures/distribution_target_curve_20190522_sky_sat_i_38lf.png}
    %\vspace{0.01\baselineskip}
\end{minipage}

%\vspace{-1.2\baselineskip}
\caption{Probabilistic prediction curves for different input data (22/05/2019):  sky images, satellite observations and extra irradiance channels (IC). Without the exrta IC (left column), the model based on satellite images only (first raw) outputs the most uncertain predictions, the 5-95\% quantile area ranging from 200 to 1000 W/$\text{m}^2$. Adding an additional IC appears to narrow the predicted uncertainty in the first two setups (sky or satellite images). In addition, models trained on sky images (with or without satellite images or IC) provide the most accurate very short-term prediction (10-min ahead).}

\label{fig:uncertainties_comparisons_2}
\end{figure*}

